When Safe Models Merge into Danger: Exploiting Latent Vulnerabilities in LLM Fusion

Model merging has emerged as a powerful technique for combining specialized capabilities from multiple fine-tuned LLMs without additional training costs. However, the security implications of this widely-adopted practice remain critically underexplored. In this work, we reveal that model merging introduces a novel attack surface that can be systematically exploited to compromise safety alignment. We present TrojanMerge,, a framework that embeds latent malicious components into source models that remain individually benign but produce severely misaligned models when merged. Our key insight is formulating this attack as a constrained optimization problem: we construct perturbations that preserve source model safety through directional consistency constraints, maintain capabilities via Frobenius directional alignment constraints, yet combine during merging to form pre-computed attack vectors. Extensive experiments across 9 LLMs from 3 model families demonstrate that TrojanMerge, consistently achieves high harmful response rates in merged models while source models maintain safety scores comparable to unmodified versions. Our attack succeeds across diverse merging algorithms and remains effective under various hyperparameter configurations. These findings expose fundamental vulnerabilities in current model merging practices and highlight the urgent need for security-aware mechanisms.

==> Figures/dare_sensitivity.tex <==
\begin{figure}[!ht]
    \centering
    \begin{tikzpicture}
    \begin{axis}[
        width=0.8\linewidth,
        height=6cm,
        xlabel={DARE Pruning Rate $p$},
        ylabel={Performance (HS\%)},
        xmin=0.1, xmax=0.9,
        ymin=0, ymax=100,
        xtick={0.2,0.4,0.6,0.8},
        grid=both,
        grid style={line width=.1pt, draw=gray!10},
        major grid style={line width=.2pt,draw=gray!25},
        legend style={
            at={(0.5,-0.25)},
            anchor=north,
            legend columns=3,
            cells={anchor=west}
        },
        tick label style={font=\small},
        label style={font=\small},
        legend style={font=\small}
    ]
    
    % Llama 2 data
    \addplot[color=blue, mark=*, mark size=2, thick] coordinates {
        (0.2, 76.9)
        (0.4, 67.3)
        (0.6, 20.0)
        (0.8, 13.1)
    };
    \addlegendentry{Llama 2}
    
    % Llama 3 data
    \addplot[color=red, mark=square*, mark size=2, thick] coordinates {
        (0.2, 78.1)
        (0.4, 56.9)
        (0.6, 56.9)
        (0.8, 14.2)
    };
    \addlegendentry{Llama 3}
    
    % Mistral data
    \addplot[color=green, mark=triangle*, mark size=2, thick] coordinates {
        (0.2, 80.1)
        (0.4, 68.1)
        (0.6, 63.1)
        (0.8, 70.0)
    };
    \addlegendentry{Mistral}
    
    \end{axis}
    \end{tikzpicture}
    \caption{Impact of DARE Pruning Rate $p$ on \name's Performance Across Different LLMs (\texttt{AdvBench}, HS\%). Higher values indicate more effective attacks.}
    \label{fig:dare_sensitivity}
\end{figure}

==> Figures/scaling_sensitivity.tex <==
\begin{figure}[!ht]
    \centering
    \begin{tikzpicture}
    \begin{axis}[
        width=0.8\linewidth,
        height=6cm,
        xlabel={Scaling Factor $\lambda$},
        ylabel={Performance (HS\%)},
        xmin=0.1, xmax=1.1,
        ymin=0, ymax=100,
        xtick={0.2,0.4,0.6,0.8,1.0},
        grid=both,
        grid style={line width=.1pt, draw=gray!10},
        major grid style={line width=.2pt,draw=gray!25},
        legend style={
            at={(0.5,-0.25)},
            anchor=north,
            legend columns=3,
            cells={anchor=west}
        },
        tick label style={font=\small},
        label style={font=\small},
        legend style={font=\small}
    ]
    
    % Llama 2 data
    \addplot[color=blue, mark=*, mark size=2, thick] coordinates {
        (0.2, 1.0)
        (0.4, 1.0)
        (0.6, 14.0)
        (0.8, 44.0)
        (1.0, 71.9)
    };
    \addlegendentry{Llama 2}
    
    % Llama 3 data
    \addplot[color=red, mark=square*, mark size=2, thick] coordinates {
        (0.2, 6.0)
        (0.4, 20.0)
        (0.6, 58.1)
        (0.8, 74.0)
        (1.0, 81.4)
    };
    \addlegendentry{Llama 3}
    
    % Mistral data
    \addplot[color=green, mark=triangle*, mark size=2, thick] coordinates {
        (0.2, 28.1)
        (0.4, 35.2)
        (0.6, 51.0)
        (0.8, 66.2)
        (1.0, 85.4)
    };
    \addlegendentry{Mistral}
    
    \end{axis}
    \end{tikzpicture}
    \caption{Impact of Scaling Factor $\lambda$ on \name's Performance Across Different LLMs (\texttt{AdvBench}, HS\%). Higher values indicate more effective attacks.}
    \label{fig:scaling_sensitivity}
\end{figure}

==> Figures/ties_topk_sensitivity.tex <==
\begin{figure}[!ht]
    \centering
    \begin{tikzpicture}
    \begin{axis}[
        width=0.8\linewidth,
        height=6cm,
        xlabel={TIES-Merging Top-K Parameter $K$},
        ylabel={Performance (HS\%)},
        xmin=5, xmax=55,
        ymin=0, ymax=95,
        xtick={10,20,30,40,50},
        grid=both,
        grid style={line width=.1pt, draw=gray!10},
        major grid style={line width=.2pt,draw=gray!25},
        legend style={
            at={(0.5,-0.25)},
            anchor=north,
            legend columns=3,
            cells={anchor=west}
        },
        tick label style={font=\small},
        label style={font=\small},
        legend style={font=\small}
    ]
    
    % Llama 2 data
    \addplot[color=blue, mark=*, mark size=2, thick] coordinates {
        (10, 58.1)
        (20, 51.0)
        (30, 55.2)
        (40, 56.9)
        (50, 66.0)
    };
    \addlegendentry{Llama 2}
    
    % Llama 3 data
    \addplot[color=red, mark=square*, mark size=2, thick] coordinates {
        (10, 56.0)
        (20, 76.0)
        (30, 79.0)
        (40, 85.0)
        (50, 88.1)
    };
    \addlegendentry{Llama 3}
    
    % Mistral data
    \addplot[color=green, mark=triangle*, mark size=2, thick] coordinates {
        (10, 76.0)
        (20, 81.7)
        (30, 84.0)
        (40, 83.1)
        (50, 83.1)
    };
    \addlegendentry{Mistral}
    
    \end{axis}
    \end{tikzpicture}
    \caption{Impact of TIES-Merging Top-K Parameter $K$ on \name's Performance Across Different LLMs (\texttt{AdvBench}, HS\%). Higher values indicate more effective attacks.}
    \label{fig:ties_topk_sensitivity}
\end{figure}

==> Figures/weighting_factor_sensitivity.tex <==
\begin{figure}[!ht]
    \centering
    
    % 第一行：Scaling Factor 和 Weighting Factor
    \begin{subfigure}{0.48\textwidth}
        \centering
        \begin{tikzpicture}
        \begin{axis}[
            width=\linewidth,
            height=5cm,
            xlabel={Scaling Factor $\lambda$},
            ylabel={Performance (HS\%)},
            xmin=0.1, xmax=1.1,
            ymin=0, ymax=100,
            xtick={0.2,0.4,0.6,0.8,1.0},
            grid=both,
            grid style={line width=.1pt, draw=gray!10},
            major grid style={line width=.2pt,draw=gray!25},
            % 移除图例设置
            tick label style={font=\small},
            label style={font=\small},
        ]
        
        % Llama 2 data
        \addplot[color=blue, mark=*, mark size=1.5, thick] coordinates {
            (0.2, 1.0)
            (0.4, 1.0)
            (0.6, 14.0)
            (0.8, 44.0)
            (1.0, 71.9)
        };
        % 移除 \addlegendentry
        
        % Llama 3 data
        \addplot[color=red, mark=square*, mark size=1.5, thick] coordinates {
            (0.2, 6.0)
            (0.4, 20.0)
            (0.6, 58.1)
            (0.8, 74.0)
            (1.0, 81.4)
        };
        % 移除 \addlegendentry
        
        % Mistral data
        \addplot[color=green, mark=triangle*, mark size=1.5, thick] coordinates {
            (0.2, 28.1)
            (0.4, 35.2)
            (0.6, 51.0)
            (0.8, 66.2)
            (1.0, 85.4)
        };
        % 移除 \addlegendentry
        
        \end{axis}
        \end{tikzpicture}
        \caption{Scaling Factor $\lambda$}
        \label{fig:scaling_sensitivity}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.48\textwidth}
        \centering
        \begin{tikzpicture}
        \begin{axis}[
            width=\linewidth,
            height=5cm,
            xlabel={Weighting Factor $x$},
            ylabel={Performance (HS\%)},
            xmin=0.55, xmax=0.95,
            ymin=0, ymax=100,
            xtick={0.6,0.7,0.8,0.9},
            grid=both,
            grid style={line width=.1pt, draw=gray!10},
            major grid style={line width=.2pt,draw=gray!25},
            % 移除图例设置
            tick label style={font=\small},
            label style={font=\small},
        ]
        
        % Llama 2 data
        \addplot[color=blue, mark=*, mark size=1.5, thick] coordinates {
            (0.6, 64.0)
            (0.7, 51.0)
            (0.8, 20.0)
            (0.9, 15.0)
        };
        % 移除 \addlegendentry
        
        % Llama 3 data
        \addplot[color=red, mark=square*, mark size=1.5, thick] coordinates {
            (0.6, 85.0)
            (0.7, 56.0)
            (0.8, 29.0)
            (0.9, 21.0)
        };
        % 移除 \addlegendentry
        
        % Mistral data
        \addplot[color=green, mark=triangle*, mark size=1.5, thick] coordinates {
            (0.6, 84.8)
            (0.7, 70.0)
            (0.8, 66.0)
            (0.9, 46.9)
        };
        % 移除 \addlegendentry
        
        \end{axis}
        \end{tikzpicture}
        \caption{Weighting Factor $x$}
        \label{fig:weighting_factor_sensitivity}
    \end{subfigure}
    
    % 第二行：DARE Pruning Rate 和 TIES Top-K Parameter
    \begin{subfigure}{0.48\textwidth}
        \centering
        \begin{tikzpicture}
        \begin{axis}[
            width=\linewidth,
            height=5cm,
            xlabel={DARE Pruning Rate $p$},
            ylabel={Performance (HS\%)},
            xmin=0.1, xmax=0.9,
            ymin=0, ymax=100,
            xtick={0.2,0.4,0.6,0.8},
            grid=both,
            grid style={line width=.1pt, draw=gray!10},
            major grid style={line width=.2pt,draw=gray!25},
            % 移除图例设置
            tick label style={font=\small},
            label style={font=\small},
        ]
        
        % Llama 2 data
        \addplot[color=blue, mark=*, mark size=1.5, thick] coordinates {
            (0.2, 76.9)
            (0.4, 67.3)
            (0.6, 20.0)
            (0.8, 13.1)
        };
        % 移除 \addlegendentry
        
        % Llama 3 data
        \addplot[color=red, mark=square*, mark size=1.5, thick] coordinates {
            (0.2, 78.1)
            (0.4, 56.9)
            (0.6, 56.9)
            (0.8, 14.2)
        };
        % 移除 \addlegendentry
        
        % Mistral data
        \addplot[color=green, mark=triangle*, mark size=1.5, thick] coordinates {
            (0.2, 80.1)
            (0.4, 68.1)
            (0.6, 63.1)
            (0.8, 70.0)
        };
        % 移除 \addlegendentry
        
        \end{axis}
        \end{tikzpicture}
        \caption{DARE Pruning Rate $p$}
        \label{fig:dare_sensitivity}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.48\textwidth}
        \centering
        \begin{tikzpicture}
        \begin{axis}[
            width=\linewidth,
            height=5cm,
            xlabel={TIES-Merging Top-K Parameter $K$},
            ylabel={Performance (HS\%)},
            xmin=5, xmax=55,
            ymin=0, ymax=95,
            xtick={10,20,30,40,50},
            grid=both,
            grid style={line width=.1pt, draw=gray!10},
            major grid style={line width=.2pt,draw=gray!25},
            % 移除图例设置
            tick label style={font=\small},
            label style={font=\small},
        ]
        
        % Llama 2 data
        \addplot[color=blue, mark=*, mark size=1.5, thick] coordinates {
            (10, 58.1)
            (20, 51.0)
            (30, 55.2)
            (40, 56.9)
            (50, 66.0)
        };
        % 移除 \addlegendentry
        
        % Llama 3 data
        \addplot[color=red, mark=square*, mark size=1.5, thick] coordinates {
            (10, 56.0)
            (20, 76.0)
            (30, 79.0)
            (40, 85.0)
            (50, 88.1)
        };
        % 移除 \addlegendentry
        
        % Mistral data
        \addplot[color=green, mark=triangle*, mark size=1.5, thick] coordinates {
            (10, 76.0)
            (20, 81.7)
            (30, 84.0)
            (40, 83.1)
            (50, 83.1)
        };
        % 移除 \addlegendentry
        
        \end{axis}
        \end{tikzpicture}
        \caption{TIES-Merging Top-K Parameter $K$}
        \label{fig:ties_topk_sensitivity}
    \end{subfigure}
    
    % 在主图标题下方添加共享图例
    \vspace{0.5cm}
    \begin{tikzpicture}
    \begin{axis}[
        hide axis,
        xmin=0, xmax=1,
        ymin=0, ymax=1,
        legend style={
            at={(0.5,0.5)},
            anchor=center,
            legend columns=3,
            cells={anchor=west},
            font=\small
        }
    ]
    \addlegendimage{color=blue, mark=*, mark size=1.5, thick}
    \addlegendentry{Llama 2}
    \addlegendimage{color=red, mark=square*, mark size=1.5, thick}
    \addlegendentry{Llama 3}
    \addlegendimage{color=green, mark=triangle*, mark size=1.5, thick}
    \addlegendentry{Mistral}
    \end{axis}
    \end{tikzpicture}
    \vspace{0.3cm}
    
    \caption{Impact of Different Hyperparameters on \name's Performance Across Different LLMs (\texttt{AdvBench}, HS\%). Higher values indicate more effective attacks. (a) Scaling Factor $\lambda$ controls the magnitude of parameter adjustments. (b) Weighting Factor $x$ balances the influence of different model components. (c) DARE Pruning Rate $p$ determines the proportion of parameters pruned during merging. (d) TIES-Merging Top-K Parameter $K$ controls the number of top parameters retained during merging.}
    \label{fig:hyperparameter_sensitivity}
\end{figure}
